Resilience of Well-structured Graph Transformation Systems

Resilience is a concept of rising interest in computer science and software engineering. For systems in which correctness w.r.t. a safety condition is unachievable, fast recovery is demanded. We investigate resilience problems of graph transformation systems. Our main contribution is the decidability of two resilience problems for well-structured graph transformation systems (with strong compatibility). We prove our results in the abstract framework of well-structured transition systems and apply them to graph transformation systems, incorporating also the concept of adverse conditions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{69}
\providecommand{\publicationstatus}{B. Hoffmann and M. Minas (Eds.): Twelfth International\\ Workshop on Graph Computation Models (GCM 2021)\\
EPTCS 350, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.350.5}{10.4204/EPTCS.350.5}}

